Vehicle Following On A Ring Road Under Safety Constraints: Role of Connectivity and Coordination

A fundamental problem in traffic networks is driving under safety and limited physical space constraints. In this paper, we design longitudinal vehicle controllers and study the dynamics of a system of homogeneous vehicles on a single-lane ring road in order to understand the interplay of limited space, speed, and safety. Each vehicle in the system either operates in the cruise control mode or follows a vehicle ahead by keeping a safe time headway. We show that if the number of vehicles is less than a certain critical threshold, vehicles can occupy the limited space in many different configurations, i.e., different platoons of different sizes, and they converge to a uniform maximum speed while attenuating errors in the relative spacing upstream a platoon. If the number of vehicles exceeds the threshold, vehicles converge to a unique symmetric configuration and the equilibrium speed decreases as the number of vehicles increases. Next, we consider vehicle-to-vehicle (V2V) communication and show that it increases the critical number of vehicles that can travel with the maximum speed. Finally, we consider central coordination and show that the proposed controllers can force vehicles to converge to a desired configuration specified by the coordinator while maintaining safety and comfort. We demonstrate the performance of the proposed controllers via simulation.

==> arXiv_Prelim_IV20.tex <==
\section{Background And Preliminaries}\label{Section: Prelim and background}
\subsection{Preliminaries}
In this section, we first formally define the terminologies that are going to be used during the rest of the paper. We then review relevant results from \cite{Ioannou.Chien.1993} for a platoon of vehicles on a single lane road without explicit spacing constraint.
\par
Consider an interconnected dynamical system with $n$ agents, e.g., see Figure \ref{Fig: InterconnectedSys}. Assume that the dynamics of the system is described by,
\begin{equation}\label{Eq: Motion of platoon}
\begin{split}
%   \dot{z}_i & = f_i(t, z_i, z_{i+1}), \:\: i = 1, 2, \cdots, n-1   \\
%   \dot{z}_n & = f_n(t,z_n), \:\: z(t_0) = z_{init}
   \dot{z}_i & = f_i(z_i, z_{i+1}), \:\: i = 1, 2, \cdots, n-1  \\
   \dot{z}_n & = f_n(z_n), \:\: z(0) \in D \\
   y_i &= c^T_iz_i, \:\: i = 1, 2, \cdots, n, \:\: 
\end{split}
\end{equation}
where $z_i \in \mathbb{R}^m$ is the vector of states of the $i^{th}$ agent, $z^T = \begin{pmatrix}
                                                                                   z^T_1 & z^T_2 & \cdots & z^T_n
                      \end{pmatrix}$,
%                      \ksmargin{special case or generalization?}
$f_i: D \rightarrow \mathbb{R}^m$ is Lipschitz continuous in $z$ on $D$, where $D$ is a domain of interest that contains $z(0)$, $c_i \in \mathbb{R}^m$ is a constant vector, and $y_i$ is the $i^{th}$ output, $i = 1, 2, \cdots, n$. A generalization of \eqref{Eq: Motion of platoon} is when the $n^{th}$ agent is interconnected back to the first agent, i.e., $\dot{z}_n = f_n(z_n, z_{1})$. As an example, let \eqref{Eq: Motion of platoon} describe the motion of a platoon of $n$ vehicles, where the vehicle numbered $n$ is the leader and all other vehicles are followers. Then, for $i = 1, 2, \cdots, n-1$, $z_i$ can consist of the relative spacing, speed, and acceleration of the $i^{th}$ vehicle, $z_n$ can consist of the speed and acceleration of the leader, and $y_i$ can be the acceleration of the $i^{th}$ vehicle, $i = 1, 2, \cdots, n$. 
\par
We have assumed in \eqref{Eq: Motion of platoon} that the external input to the system is a function of the states of the system. Therefore, it is not explicitly present.
\begin{figure}[H]
\centering
\includegraphics[width=0.6\textwidth]{Figures/InterconnectedSys.png}
\vspace*{2mm}
\caption{\sf \mpcomment{An interconnected dynamical system with $n$ agents with arrows indicating the flow of information}}\label{Fig: InterconnectedSys}
\end{figure}\ksmargin{maybe explain $z_{i+1}$ on arrow in the caption}
\begin{definition}\label{Def: equilibrium}
\textbf{(Equilibrium)} An equilibrium state of the system \eqref{Eq: Motion of platoon} is a state $z^{*} \in D$
such that,
\begin{equation}\label{Eq: Definition of Equilibrium}
\begin{split}
%    f_i(t,z^{*}_{i}, z^{*}_{i+1}) & = 0, \:\: i = 1, 2, \cdots, n-1 \\
%    f_n(t,z^{*}_{n}) & = 0
    f_i(z^{*}_{i}, z^{*}_{i+1}) & = 0, \:\: i = 1, 2, \cdots, n-1 \\
    f_n(z^{*}_{n}) & = 0
\end{split}
\end{equation}
\par
In other words, if the system starts from the state $z^{*}$ at some time $t \geq 0$, it remains in that state for all future times.
\end{definition}
Let $z(t;z(0))$ denote the solution to \eqref{Eq: Motion of platoon}. The following stability definitions are adopted from \cite{ioannou2012robust}.
\begin{definition}
\textbf{(Stability)} An equilibrium state $z^{*}$ of the interconnected dynamical system \eqref{Eq: Motion of platoon} is \par
%$(i)$ \emph{stable (in the sense of Lyapunov)} if for arbitrary $t_0$ and $\epsilon > 0$ there exists a $\delta(\epsilon,t_0) > 0$ such that $\|z_{init} - z^{*}\| < \delta(t_0,\epsilon)$ implies $\|z(t;t_0,z_{init}) - z^{*}\| < \epsilon$ for all $t \geq t_0$ \par
$(i)$ \emph{stable (in the sense of Lyapunov)} if for every $\epsilon > 0$ there exists a $\delta(\epsilon) > 0$ such that $\|z(0) - z^{*}\| < \delta(\epsilon)$ implies $\|z(t;z(0)) - z^{*}\| < \epsilon$ for all $t \geq 0$ \par
%$(ii)$ \emph{uniformly stable} if it is stable and if $\delta(\epsilon,t_0)$ in $(i)$ is independent of $t_0$ \par
%$(iii)$ \emph{asymptotically stable} if it is stable, and there exists a $\delta(t_0) > 0$ such that $\|z_{init} - z^{*}\| < \delta(t_0)$ implies $lim_{t \rightarrow \infty} \|z(t;t_0,z_{init}) - z^{*}\| = 0$. If this condition holds for every positive $\delta(t_0)$, then the equilibrium is globally asymptotically stable \par
$(ii)$ \emph{asymptotically stable} if it is stable, and there exists a $\delta > 0$ such that $\|z(0) - z^{*}\| < \delta$ implies $lim_{t \rightarrow \infty} \|z(t;z(0)) - z^{*}\| = 0$. If this condition holds for every positive $\delta$, then the equilibrium is globally asymptotically stable \par
%$(iv)$ \emph{Uniformly Asymptotically Stable (UAS)} if it is uniformly stable, and for every $t_0 \in [0, \infty)$ and $\epsilon > 0$, there exists a $\delta_0 > 0$ independent of $t_0$ and $\epsilon$ and a $T(\epsilon) > 0$ independent of $t_0$ such that $\|z(t;t_0,z_{init}) - z^{*}\| < \epsilon$ for all $t \geq t_0 + T(\epsilon)$ whenever $\|z_{init} - z^{*}\|< \delta_0$ \par
%$(v)$ \emph{Globally Uniformly Asymptotically Stable (GUAS)} if it is uniformly stable, and for each $\delta_0 > 0$ and $\epsilon > 0$, there exists $T(\epsilon, \delta_0) > 0$ such that $\|z(t;t_0,z_{init}) - z^{*}\| < \epsilon$ for all $t \geq t_0 + T(\epsilon, \delta_0)$ whenever $\|z_{init} - z^{*}\|< \delta_0$ \par
%$(vi)$ \emph{Uniformly Exponentially Stable (UES)} if there exists an $\alpha > 0$, and for arbitrary $\epsilon > 0$ there exists a $\delta(\epsilon) > 0$ such that $\|z_{init} - z^{*}\| < \delta(\epsilon)$ implies,
%\begin{equation*}\label{Eq: Exponential stability}
%  \|z(t;t_0,z_{init}) - z^{*}\| < \epsilon e^{-\alpha(t - t_0)}, \:\: \forall t \geq t_0
%\end{equation*}
$(iii)$ \emph{exponentially stable} if there exists an $\alpha > 0$, and for every $\epsilon > 0$ there exists a $\delta(\epsilon) > 0$ such that $\|z(0)- z^{*}\| < \delta(\epsilon)$ implies,
\begin{equation*}\label{Eq: Exponential stability}
  \|z(t;z(0)) - z^{*}\| < \epsilon e^{-\alpha t}, \:\: \forall t \geq 0
\end{equation*}
\par 
If this condition holds for all $\delta(\epsilon) > 0$, then the equilibrium is globally exponentially stable.
\end{definition}
\ksmargin{need to use this earlier to motivate this subsection}
%\ksmargin{also exponential}
Note that asymptotic and exponential stability of an equilibrium are steady state performance measures of the system. Another important aspect in interconnected dynamical systems is the transient performance. \mpcomment{For example, in a platoon of vehicles, errors in the desired inter-vehicle spacing, speed, or acceleration may amplify during the transient as one goes upstream the platoon \cite{Sheikholeslam:M91/115,Ioannou.Chien.1993,hedrick1991longitudinal}, even when all signals converge exponentially fast to zero. In the literature of platoon studies, the term “string stability” is used to describe this transient phenomenon, also known as \emph{slinky effect}. In order to distinguish from stability (in the sense of Lyapunov), we use the term “string attenuation” defined as follows.}
%Without loss of generality, assume that $Z_0 = 0$.
%Consider the interconnected dynamical system \eqref{Eq: Motion of platoon}. For $i = 1, 2, \cdots, n$, let $y_i = c^T_iz_i$, where $c_i \in \mathbb{R}^m$ is a constant vector.
%and $y^T = \begin{pmatrix}                                 y^T_1 & y^T_2 & \cdots & y^T_{n}
%                      \end{pmatrix}$.
%Assume that there is a \kscomment{small} perturbation in $y_n$ at $t = 0$. \ksmargin{what does 'small' mean? Overall, Def 3 needs rewriting}
\begin{definition}
\textbf{(String Attenuation)} 
Let $y^T = \begin{pmatrix} y_1 & y_2 & \cdots & y_n \end{pmatrix}$ and assume that $y \in \mathcal{L}_2$. We say that the interconnected dynamical system \eqref{Eq: Motion of platoon} is \emph{string attenuated in the $\mathcal{L}_2$ sense} with respect to $y$ if for $i = 1,2, \cdots, n-1$, there exists a nonnegative constant $\gamma_i$ such that $\|y_i\|_{\mathcal{L}_{2}} \leq \|y_{i+1}\|_{\mathcal{L}_{2}} + \gamma_i$. Moreover, assume that $y$ is uniformly bounded. We say that the system is \emph{string attenuated in the $\mathcal{L}_\infty$ sense} with respect to $y$ if for $i = 1,2, \cdots, n-1$, there exists a nonnegative constant $\gamma_i$ such that $\|y_i\|_{\mathcal{L}_{\infty}} \leq \|y_{i+1}\|_{\mathcal{L}_{\infty}} + \gamma_i$.
\end{definition}
%\mpcomment{\begin{remark}
%It can be shown that string attenuation in the $\mathcal{L}_\infty$ sense implies string attenuation in the $\mathcal{L}_2$ sense, while the converse is not true.
%\end{remark}}
\begin{remark}
Assume that for $i = 1, 2, \cdots, n$, $f_i$ in \eqref{Eq: Motion of platoon} is linear in $z$. We can write the dynamics of \eqref{Eq: Motion of platoon} as the following LTI system,
\begin{equation}\label{Eq: LTI interconnected system}
    \begin{aligned}
    \dot{z} &= A z, \:\: z(0) \in D \\
    y_i &= c^{T}_iz_i, \:\: i = 1, 2, \cdots, n
    \end{aligned}
\end{equation}
where,
\begin{equation*}
    A = \begin{pmatrix}
            A_{1} & B_{1} & 0 & \cdots & 0 \\
            0 & A_{2} & B_{2} & \cdots & 0 \\
            \vdots & \vdots & \vdots & \ddots & \vdots \\
            0 & 0 & 0 & \cdots & A_{n} \\
    \end{pmatrix}
\end{equation*}
in which all zeros are $m \times m$ submatrices, $A_i \in \mathbb{R}^{m \times m}$, $i = 1, 2, \cdots, n$, and $B_i \in \mathbb{R}^{m \times m}$, $i = 1, 2, \cdots, n-1$ are constant matrices. The trivial equilibrium $z^{*} = 0$ of \eqref{Eq: LTI interconnected system} is globally exponentially stable if and only if all eigenvalues of $A$ fall in the open left half of the complex plane. Without loss of generality, let $z_i(0) = 0$, $i = 1, 2, \cdots, n-1$. 
%\ksmargin{are you trying to say that $G_i$ can be written explicitly in terms of $A$ and $c$; if so, say it explicitly}
Assume that by taking Laplace transform from \eqref{Eq: LTI interconnected system}, the following relationship can be found,
\begin{equation*}\label{Eq: yi = Li yi+1}
 Y_i(s) = G_i(s) Y_{i+1}(s), \:\: i = 1,2,\cdots, n-1
\end{equation*}
where $Y_i(s)$ is the Laplace transform of $y_i$ and $G_i(s)$ is the frequency domain transfer function. The string attenuation property in the $\mathcal{L}_2$ sense with respect to $y$ is then equivalent to $|G_i(j\omega)| \leq 1$, $\forall \omega \geq 0$, $i = 1, 2, \cdots, n-1$. Additionally, assume that for $i = 1, 2, \cdots, n$, $y$ is uniformly bounded. A sufficient condition for string attenuation in the $\mathcal{L}_\infty$ sense with respect to $y$ is $\|g_i\|_{\mathcal{L}_{1}} \leq 1$, where $g_i(t)$ is the impulse response of $G_i(s)$, $i = 1, 2, \cdots, n-1$.
\end{remark}
\subsection{Results for No Space Constraint}\label{Subsection: Review of results for line}
We provide a brief summary of relevant results \cite{Ioannou.Chien.1993}, when space constraint is not explicitly considered. Consider again a platoon of $n$ vehicles where the vehicle numbered $n$ is the leader. For $i = 1, 2, \cdots, n$, let $x_i(t)$ denote the distance of the $i^{th}$ vehicle with respect to a fixed reference point on the roadside, and $v_i(t)$, $a_i(t)$ denote its instantaneous speed and acceleration at time $t \geq 0$, respectively. In the rest of the paper, except when needed, we use $x_i$, $v_i$, and $a_i$ without explicitly mentioning their dependence on time. Assuming that the road surface is horizontal and there is no wind gust, we can use Newton's second law of motion for vehicle $i$, $i = 1,2, \cdots, n$, to write,
\begin{equation*}\label{Eq: (Acceleration Control)Newton's second law of motion}
  m_ia_i = F_i - k_{d_i}v^2_i - d_{m_i}(v_i)
\end{equation*}
where $F_i$ is the engine force, $m_i$ is the mass, $k_{d_i}$ is the aerodynamic drag coefficient, and $d_{m_i}(v_i)$ is the mechanical friction of the $i^{th}$ vehicle travelling with the speed $v_i$ \cite{CAUDILL1976195}. We consider a first-order engine dynamics,
\begin{equation*}\label{Eq: (Acceleration Control)Engine dynamics}
  \dot{F}_i = \frac{1}{\tau_i(v_i)}(u_i - F_i)
\end{equation*}
where $u_i$ is the throttle input to the engine, and $\tau_i(v_i)$ is the engine's time constant at the speed $v_i$ \cite{Sheikholeslam:M91/115}. This simple engine dynamics is reported to be useful in platoon studies \cite{Sheikholeslam:M91/115}. By combining the last two equations we derive,
\begin{equation} \label{Eq: Vehicle model} 
%\begin{align}
%  \frac{d}{dt}x_i &= \dot{x}_i, \label{Eq:(Acceleration Control)Speed dynamics for vehicle i} \\
%  \frac{d}{dt}\dot{x}_i &= \ddot{x}_i \label{Eq:(Acceleration Control)Acceleration dynamics for vehicle i}\\
  \dot{a}_i = \beta(v_i,a_i) + \alpha(v_i)u_i %+ d_i %\label{Eq:(Acceleration Control)Jerk dynamics for vehicle i}
%\end{align}
\end{equation}
where,
%\ksmargin{expressions for $\alpha$ and $\beta$ seem to have typos: $\alpha$ should have a minus, $\beta$ should have derivative of $d_{m_i}(v_i)$, etc.}
\begin{equation*}\label{Eq: (Acceleration Control)alpha(v_i)}
\begin{split}
   \alpha(v_i)  & = \frac{1}{m_i \tau_i(v_i)} \\
    \beta(v_i,a_i)  & = -2\frac{k_{d_i}}{m_i}v_i a_i - \frac{1}{m_i}\dot{d}_{m_i}(v_i) - \frac{1}{\tau_i(v_i)}[a_i + \frac{k_{d_i}}{m_i} v^2_i + \frac{d_{m_i}(v_i)}{m_i}]
\end{split}
\end{equation*}
%and $d_i$ accounts for unmodelled dynamics and external disturbance.\par
\par
At each speed $v_i$, the following nonlinear controller \cite{Ioannou.Chien.1993} linearizes the vehicle dynamics described by \eqref{Eq: Vehicle model},
\begin{equation}\label{Eq: (Acceleration Control)(Time) nonlinear feedback of u_i}
    u_i = \frac{1}{\alpha(v_i)}[c_i - \beta(v_i,a_i)]
\end{equation}
where $c_i$ is a feedback controller to be designed. By substituting \eqref{Eq: (Acceleration Control)(Time) nonlinear feedback of u_i} into \eqref{Eq: Vehicle model}, the nonlinear terms cancel out and we derive the following simplified vehicle dynamics,
\begin{equation} \label{Eq: Simplified Vehicle dynamics} 
\dot{a}_i = c_i %+ d_i
\end{equation}
%Let $d_i \equiv 0$, $i = 1,2, \cdots, n$.
\par
For $i = 1, 2, \cdots, n-1$, let $y_i = x_{i+1} - x_i$ denote the relative spacing, and $\delta_i = y_i - (hv_i + S_0)$ the error in the desired relative spacing, where $S_0 > 0$ is a constant and $h$ is the time headway constant. The time headway constant is chosen such that two consecutive vehicles do not collide under a worst-case stopping scenario. An instance of such a scenario is when vehicle $i+1$ is decelerating at maximum deceleration while its predecessor, i.e., vehicle $i$, is accelerating at maximum acceleration, while the two vehicles were travelling with approximately the same speed \cite{Ioannou.Chien.1993}. Choosing the value of $h$ according to this scenario ensures no rear-end collision if vehicle $i$ obeys the safety rule $\delta_i(0) \geq 0$. The minimum safe value of $h = 0.3 \: [s]$ is reported in \cite{Ioannou.Chien.1993} for realistic vehicle dynamics.  \par
%\ksmargin{where $C_p$, $C_n$ and $K_a$ are control parameters}
For the follower vehicles of the platoon, i.e., $i = 1, 2, \cdots, n-1$, the feedback controller $c_i$ can be designed as follows \cite{Ioannou.Chien.1993},
\begin{equation}\label{Eq: (Acceleration Control)(Time)(IoannouChien) linear feedback of u_i}
c_i = C_{p}\delta_i + C_{v}\dot{\delta}_i + K_a a_i
\end{equation}
%Let $z^T_i = \begin{pmatrix}                                                       \delta_i & \dot{\delta}_i & \ddot{\delta}_i
%\end{pmatrix}$,
%$z^T_n = \begin{pmatrix}
%     v_n - v_{d} & a_n
%     \end{pmatrix}$,
%and $Z^T = \begin{pmatrix}                               z^T_1 & z^T_2 & \cdots & z^T_n                          \end{pmatrix}$,
%where $v_{d}$ is the desired speed trajectory for the lead vehicle.
%Let $V_d$ be the constant desired speed for the lead vehicle, i.e., vehicle numbered $n$,
where $C_p, C_v > 0$, $K_a < 0$ are design parameters. Let $G(s)$ be the frequency domain transfer function between $\delta_i$ and $\delta_{i+1}$, and $g(t)$ be the impulse response. By substituting $c_i$ in \eqref{Eq: (Acceleration Control)(Time)(IoannouChien) linear feedback of u_i} into \eqref{Eq: Simplified Vehicle dynamics}, the closed loop system becomes LTI. 
%with $\begin{pmatrix} \delta_i & \dot{\delta}_i & a_i \end{pmatrix} = \begin{pmatrix} 0 & 0 & 0 \end{pmatrix}$, $i = 1,2, \cdots, n-1$, $\begin{pmatrix} v_n - V_d & a_n \end{pmatrix} = \begin{pmatrix} 0 & 0 \end{pmatrix}$ as its unique equilibrium. Assuming that $\begin{pmatrix} v_n - V_d & a_n \end{pmatrix} \rightarrow \begin{pmatrix} 0 & 0 \end{pmatrix}$ as $t \rightarrow \infty$,
For desired steady state performance, i.e., desired relative spacing and desired speed, the necessary and sufficient condition is that poles of $G(s)$ lie in the open left half of the $s$-plane \cite{Ioannou.Chien.1993}. Additionally, the necessary and sufficient condition for string attenuation in the $\mathcal{L}_2$ sense with respect to $\delta_i$ is that $|G(j\omega)| \leq 1$, $\forall \omega \geq 0$. It is important to mention that, in general, $|G(j\omega)| \leq 1$, $\forall \omega \geq 0$, does not imply asymptotic stability of an equilibrium. For example, the equilibrium is unstable if $G(s) = \frac{1}{s^3 - s + 1}$. However, $|G(j\omega)| \leq 1$, $\forall \omega \geq 0$.
\par
A more desirable transient behavior in a platoon of vehicles is string attenuation in the $\mathcal{L}_\infty$ sense. Provided the asymptotic stability of the equilibrium in the above case, a sufficient condition for string attenuation in the $\mathcal{L}_\infty$ sense with respect to $\delta_i$ is $|G(j\omega)| \leq 1$, $\forall \omega \geq 0$ and $g(t) > 0$, $\forall t \geq 0$ \cite{Ioannou.Chien.1993}. As an example, the design parameters $S_o = 4 \:\: [m]$, $h = 0.4 \:\: [s]$, $C_p = 4 \:\: [\frac{1}{s^3}]$, $C_v = 28 \:\: [\frac{1}{s^2}]$, $K_a = -0.04 \:\: [\frac{1}{s}]$ satisfy the stability and string attenuation criteria \cite{Ioannou.Chien.1993}.
